Subverting Fair Image Search with Generative Adversarial Perturbations

In this work we explore the intersection fairness and robustness in the context of ranking: when a ranking model has been calibrated to achieve some definition of fairness, is it possible for an external adversary to make the ranking model behave unfairly without having access to the model or training data? To investigate this question, we present a case study in which we develop and then attack a state-of-the-art, fairness-aware image search engine using images that have been maliciously modified using a Generative Adversarial Perturbation (GAP) model. These perturbations attempt to cause the fair re-ranking algorithm to unfairly boost the rank of images containing people from an adversary-selected subpopulation. We present results from extensive experiments demonstrating that our attacks can successfully confer significant unfair advantage to people from the majority class relative to fairly-ranked baseline search results. We demonstrate that our attacks are robust across a number of variables, that they have close to zero impact on the relevance of search results, and that they succeed under a strict threat model. Our findings highlight the danger of deploying fair machine learning algorithms in-the-wild when (1) the data necessary to achieve fairness may be adversarially manipulated, and (2) the models themselves are not robust against attacks.

==> old.tex <==
\iffalse
\subsection{Subpopulation Universal Adversarial Perturbations}

\todo{need to rewrite 4.3 and 4.4}

To impact the fairness of our search engine's output, the adversary generates a perturbation that, when applied to images in the database, suppresses the ranks of members of an adversary-selected subgroup. We call this perturbation type a Subpopulation Universal Adversarial Perturbation (SUAP), and allow it to be defined for classification, regression, or ranking. We consider both \emph{targeted} and \emph{untargeted} versions of this attack (differences in their definitions are bolded for clarity).

\begin{definition}[SUAP]
A SUAP $\delta$ considers a loss function $\ell$, distribution $\mathcal{D}$ over inputs $x$, outputs $y$, subpopulations $a$, and adversary-selected subpopulation $a_s$.

An untargeted SUAP increases the loss for members of subpopulation $a_s$ while reducing the loss on other subpopulations, decreasing 
\begin{equation}
\ell_r^{\mathbf{u}}(D) = \mathbb{E}_{(x, a, y)\sim D}[\ell(x, y)|a\neq a_s] \mathbf{-} \mathbb{E}_{(x, a, y)\sim D}[\ell(x, \mathbf{y})|a=a_s].
\label{eq:untargeted}
\end{equation}

A targeted SUAP has a target output $y_t$, and pushes members of the selected subpopulation $a_s$ to the target output $y_t$, while maintaining the performance of other subpopulations, decreasing
\begin{equation}
\ell_r^{\mathbf{t}}(D) = \mathbb{E}_{(x, a, y)\sim \mathcal{D}}[\ell(x, y)|a\neq a_s] \mathbf{+} \mathbb{E}_{(x, a, y)\sim \mathcal{D}}[\ell(x, \mathbf{y_t})|a=a_s].
\label{eq:targeted}
\end{equation}

\end{definition}

\begin{table*}
\small
\centering
%\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Method} & \textbf{Loss} & \textbf{Demographic Inference} & \textbf{Fair Re-ranking}  \\ \midrule
BASE (Baseline) & None & None       & None  \\
ADV1 (Attack 1)         & $\ell_r^u$/$\ell_r^t$ & None       & None  \\
ADV1-RR (Attack 1 + Re-ranking)    & $\ell_r^u$/$\ell_r^t$ & FairFace       & DetConstSort    \\
ADV2-RR (Attack 2 + Re-ranking) & $\ell_F^u$/$\ell_F^t$ & FairFace       & DetConstSort  \\
\bottomrule
\end{tabular}%
%}
\vspace{2mm}
\caption{The four ranked lists that we compare in the study.}
\vspace{-8mm}
\label{tab:fourlists}
\end{table*}

We apply our SUAPs to the fair ranking problem. For a ranking function $f_r(D; q)$, the adversary generates a SUAP $\delta$ and applies it to the image query dataset $D$ to form $D_{\delta}=\lbrace x_i+\delta \rbrace_{i=1}^n$. If successful, the scores produced by the ranking function $s_i$ will be decreased for members of a target subpopulation, while scores outside of that subpopulation will be improved, having the effect of suppressing the adversary-selected subpopulation in the query results.

We now describe the algorithm for generating a targeted SUAP, which is similar to generating a UAP. For a goal embedding $v_q$, the attacker minimizes $\ell_r^t$ from Equation~\ref{eq:targeted}, using the inner loss function $\ell(x, y)=d(f_i(x), v_q)$. Following the UAP literature, we optimize this loss function using batch gradient descent over a validation set (independent from our test-time database $D$). For an untargeted SUAP, we simply select a query embedding $v_q$ and minimize $\ell_r^u$ from Equation~\ref{eq:untargeted}, with inner loss function $\ell(x, y)=-d(f_i(x), v_q)$.

\subsection{Attacks on Fair Re-ranking}

We consider a fair ranking-based defense for our SUAP attack. As described in \autoref{sec:detconfairface}, given the scores $s_i$ and demographics $a_i$ for images $x_i\in D$, we run a fair re-ranking on $\lbrace s_i, a_i\rbrace$ using DetConstSort \cite{geyik2019fairness}. For both the race/ethnicity and gender inference, we use the pretrained FairFace \cite{karkkainen2019fairface} classifier. We denote the gender classification model as $f_g$ and the race/ethnicity classification model as $f_e$.

Unfortunately, we demonstrate that this re-ranking procedure adds an additional vulnerability to our search engine: the demographic inference model itself may be misled, which can drastically undermine the fairness guarantees of DetConstSort, as shown in previous work \cite{ghosh2021fair}. We add two additional loss functions $\ell_g$ and $\ell_e$ to our adversarial loss function to perform this attack. The losses $\ell_g$ and $\ell_e$ attempt to mislead $f_g$ and $f_e$ on the adversary-selected demographic $a_s=(g_s, e_s)$, measured using the cross entropy loss $\ell_{XE}$:
\begin{equation}
    \ell_g(x, (g, e)) = \mathbbm{1}[g\neq g_s]\ell_{XE}(f_g(x), g)-\mathbbm{1}[g=g_s]\ell_{XE}(f_g(x), g)
\end{equation}
\begin{equation}
    \ell_e(x, (g, e)) = \mathbbm{1}[e\neq e_s]\ell_{XE}(f_e(x), e) - \mathbbm{1}[e=e_s]\ell_{XE}(f_e(x), e).
\end{equation}

We generate our SUAPs minimizing instead 
$\ell_F^t = \ell_r^t + \alpha_g\ell_g + \alpha_e\ell_e$
in the targeted case and minimizing
$\ell_F^u = \ell_r^u + \alpha_g\ell_g + \alpha_e\ell_e$ in the untargeted case. Empirically, using $\alpha_g=\alpha_e=1$ works well. Note that this strategy constructs SUAPs which target both ranking and classification models.
\fi
